Extensions of Heterogeneity in Integration and Prediction (HIP) with R Shiny Application

Multiple data views measured on the same set of participants is becoming more common and has the potential to deepen our understanding of many complex diseases by analyzing these different views simultaneously. Equally important, many of these complex diseases show evidence of subgroup heterogeneity (e.g., by sex or race). HIP (Heterogeneity in Integration and Prediction) is among the first methods proposed to integrate multiple data views while also accounting for subgroup heterogeneity to identify common and subgroup-specific markers of a particular disease. However, HIP is applicable to continuous outcomes and requires programming expertise by the user. Here we propose extensions to HIP that accommodate multi-class, Poisson, and Zero-Inflated Poisson outcomes while retaining the benefits of HIP. Additionally, we introduce an R Shiny application, accessible on shinyapps.io at https://multi-viewlearn.shinyapps.io/HIP_ShinyApp/, that provides an interface with the Python implementation of HIP to allow more researchers to use the method anywhere and on any device. We applied HIP to identify genes and proteins common and specific to males and females that are associated with exacerbation frequency. Although some of the identified genes and proteins show evidence of a relationship with chronic obstructive pulmonary disease (COPD) in existing literature, others may be candidates for future research investigating their relationship with COPD. We demonstrate the use of the Shiny application with a publicly available data. An R-package for HIP would be made available at https://github.com/lasandrall/HIP.

==> Tables/Tab_rda_grid_v_random.tex <==

\begin{table}[htbp]
    \centering
    \renewcommand{\arraystretch}{0.7}
    \caption{{\bf Number of Stable Genes and Proteins Selected by HIP (Grid)-ZIP and HIP (Random)-ZIP for the COPDGene Data.}}\label{ext:tab:rda:gridvrand}
\begin{tabular}{ccccc}
\toprule
Data & Subtype & Random & Grid & Overlap between Random and Grid\\
\midrule
 & Males & 51 & 51 & 49\\
\cmidrule{2-5}
 & Females & 50 & 50 & 47\\
\cmidrule{2-5}
\multirow[t]{-3}{*}{\centering\arraybackslash Genes} & Common & 36 & 38 & 34\\
\cmidrule{1-5}
 & Males & 20 & 20 & 20\\
\cmidrule{2-5}
 & Females & 20 & 20 & 20\\
\cmidrule{2-5}
\multirow[t]{-3}{*}{\centering\arraybackslash Proteins} & Common & 17 & 17 & 17\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_rda_num_splits.tex <==

\begin{table}[htbp]
    \centering
    \small
    \renewcommand{\arraystretch}{0.7}
    \caption{{\bf Average Number of Variables Selected Across 50 Test/Train Splits for the COPDGene Data.} Numbers shown are mean (standard deviation). Comparator methods were run without an upper bound on how many variables could be selected. HIP has no variability in the number selected because $N_top$ is specified within each split.}\label{ext:tab:rda:nsplit}
    \begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Genes} & \multicolumn{2}{c}{Proteins} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Method & Males & Females & Males & Females\\
\midrule
CVR-Poisson & 210.1 (181.2) & 311.1 (125.1) & 103.7 (90.3) & 103.7 (90.3)\\
SELPCCA-ZIP & 115.1 (168.8) & 113.4 (141.9) & 73.7 (107.2) & 73.7 (107.2)\\
Lasso-Poisson & 113.8 (28.8) & 78.8 (43.8) & 27.9 (7.3) & 27.9 (7.3)\\
Elastic Net-Poisson & 138.3 (20.5) & 103.9 (42.2) & 34.2 (6.3) & 34.2 (6.3)\\
HIP (Grid)-Poisson & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
HIP (Random)-Poisson & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
HIP (Grid)-ZIP & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
HIP (Random)-ZIP & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
HIP (Grid)-ZIP+Clinical & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
HIP (Random)-ZIP+Clinical & 125 (0) & 125 (0) & 50 (0) & 50 (0)\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_rda_num_stable.tex <==

\begin{table}[htbp]
    \centering
    \small
    \renewcommand{\arraystretch}{0.7}
    \caption{{\bf Number of Stable Genes and Proteins Selected by Method for the COPDGene Data.} The stable genes and proteins are the top 1\% of genes and proteins based on a rank determined by the number of splits the protein/gene entered the model and how many times the protein/gene was selected by the model. The 1\% is based on the 5000 genes and 2000 proteins from the unsupervised filtering.}\label{ext:tab:rda:nstable}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Genes} & \multicolumn{3}{c}{Proteins} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Method & Males & Females & Common & Males & Females & Common\\
\midrule
CVR-Poisson & 50 & 50 & 14 & 21 & 21 & 15\\
SELPCCA-ZIP & 50 & 50 & 14 & 20 & 21 & 5\\
Lasso-Poisson & 50 & 50 & 3 & 20 & 20 & 1\\
Elastic Net-Poisson & 50 & 51 & 3 & 20 & 20 & 2\\
HIP (Grid)-Poisson & 51 & 50 & 41 & 20 & 20 & 18\\
HIP (Random)-Poisson & 51 & 50 & 40 & 20 & 20 & 18\\
HIP (Grid)-ZIP & 51 & 50 & 38 & 20 & 20 & 17\\
HIP (Random)-ZIP & 51 & 50 & 36 & 20 & 20 & 17\\
HIP (Grid)-ZIP+Clinical & 50 & 50 & 33 & 20 & 20 & 18\\
HIP (Random)-ZIP+Clinical & 50 & 50 & 36 & 20 & 20 & 17\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_rda_weights_genes_F.tex <==
% Genes -  Females

\begin{table}
    \centering
    \small
    \renewcommand{\arraystretch}{0.8}
    \caption{{\bf Genes Selected by HIP (Random) for Females for the COPDGene Data.} Weights are averages from the estimated $\bm B^{d,s}$ matrices from the subset fit where the variable was selected. Higher values suggest the variable likely contributes more to association and prediction.}\label{ext:tab:rda:gene_F}
\begin{tabular}{lcc}
\toprule
ID & Symbol & Weight\\
\midrule
ENSG00000158856.18 & DMTN & 3.521\\
ENSG00000167671.12 & UBXN6 & 3.463\\
ENSG00000137216.19 & TMEM63B & 3.457\\
ENSG00000004939.15 & SLC4A1 & 3.421\\
ENSG00000130830.15 & MPP1 & 3.397\\
ENSG00000115594.12 & IL1R1 & 3.375\\
ENSG00000100325.15 & ASCC2 & 3.366\\
ENSG00000090013.11 & BLVRB & 3.357\\
ENSG00000198858.10 & R3HDM4 & 3.355\\
ENSG00000259671.1 & MTCYBP23 & 3.327\\
ENSG00000063854.13 & HAGH & 3.325\\
ENSG00000158578.21 & ALAS2 & 3.323\\
ENSG00000179262.10 & RAD23A & 3.310\\
ENSG00000137198.10 & GMPR & 3.307\\
ENSG00000101236.17 & RNF24 & 3.303\\
ENSG00000241860.7 & LOC100996442 & 3.296\\
ENSG00000073792.16 & IGF2BP2 & 3.293\\
ENSG00000135636.14 & DYSF & 3.275\\
ENSG00000141084.11 & RANBP10 & 3.245\\
ENSG00000197405.8 & C5AR1 & 3.241\\
ENSG00000102145.15 & GATA1 & 3.240\\
ENSG00000260528.5 & FAM157C & 3.226\\
ENSG00000143774.17 & GUK1 & 3.214\\
ENSG00000259600.2 & RP11\_925D83 & 3.207\\
ENSG00000197081.16 & IGF2R & 3.204\\
ENSG00000170315.14 & UBB & 3.203\\
ENSG00000287771.1 & AC007271.1 & 3.184\\
ENSG00000159346.13 & ADIPOR1 & 3.183\\
ENSG00000090238.12 & YPEL3 & 3.181\\
ENSG00000185883.12 & ATP6V0C & 3.173\\
ENSG00000251441.3 & RTEL1P1 & 3.166\\
ENSG00000259379.1 & MTND5P32 & 3.142\\
ENSG00000259626.2 & MTND3P12 & 3.136\\
ENSG00000060138.13 & YBX3 & 3.132\\
ENSG00000257335.8 & MGAM & 3.128\\
ENSG00000232334.1 & RP11\_47G112 & 3.125\\
ENSG00000137193.14 & PIM1 & 3.110\\
ENSG00000182512.5 & GLRX5 & 3.102\\
ENSG00000249138.1 & SLED1 & 3.092\\
ENSG00000234292.3 & AC123595.1 & 3.088\\
ENSG00000232528.3 & LOC100289473 & 3.085\\
ENSG00000215244.3 & LINC02649 & 3.078\\
ENSG00000135083.16 & CCNJL & 3.065\\
ENSG00000167286.10 & CD3D & 3.035\\
ENSG00000147454.14 & SLC25A37 & 2.988\\
ENSG00000084110.11 & HAL & 2.808\\
ENSG00000185031.6 & SLC2A3P2 & 2.745\\
ENSG00000258111.1 & RP11\_43D42 & 2.720\\
ENSG00000137876.11 & RSL24D1 & 2.678\\
ENSG00000271204.1 & RP11\_138A91 & 2.537\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_rda_weights_genes_M.tex <==
% Genes - Males

\begin{table}
    \centering
    \small
    \renewcommand{\arraystretch}{0.8}
    \caption{{\bf Stable Genes Selected by HIP (Random) for Males in the COPDGene Data.} Weights are averages from the estimated $\bm B^{d,s}$ matrices from the subset fit where the variable was selected. Higher values suggest the variable likely contributes more to association and prediction.}\label{ext:tab:rda:gene_M}
\begin{tabular}{lcc}
\toprule
ID & Symbol & Weight\\
\midrule
ENSG00000100325.15 & ASCC2 & 2.969\\
ENSG00000167671.12 & UBXN6 & 2.966\\
ENSG00000136842.14 & TMOD1 & 2.957\\
ENSG00000259671.1 & MTCYBP23 & 2.948\\
ENSG00000197081.16 & IGF2R & 2.932\\
ENSG00000073792.16 & IGF2BP2 & 2.902\\
ENSG00000137216.19 & TMEM63B & 2.897\\
ENSG00000101236.17 & RNF24 & 2.893\\
ENSG00000259600.2 & RP11\_925D83 & 2.880\\
ENSG00000259379.1 & MTND5P32 & 2.877\\
ENSG00000215244.3 & LINC02649 & 2.870\\
ENSG00000179262.10 & RAD23A & 2.869\\
ENSG00000198858.10 & R3HDM4 & 2.866\\
ENSG00000143774.17 & GUK1 & 2.848\\
ENSG00000158856.18 & DMTN & 2.836\\
ENSG00000287771.1 & AC007271.1 & 2.833\\
ENSG00000249138.1 & SLED1 & 2.822\\
ENSG00000137198.10 & GMPR & 2.810\\
ENSG00000259626.2 & MTND3P12 & 2.804\\
ENSG00000103342.13 & GSPT1 & 2.801\\
ENSG00000090013.11 & BLVRB & 2.798\\
ENSG00000168785.8 & TSPAN5 & 2.798\\
ENSG00000234292.3 & AC123595.1 & 2.793\\
ENSG00000130830.15 & MPP1 & 2.781\\
ENSG00000251441.3 & RTEL1P1 & 2.776\\
ENSG00000143416.21 & SELENBP1 & 2.771\\
ENSG00000197405.8 & C5AR1 & 2.769\\
ENSG00000142453.12 & CARM1 & 2.768\\
ENSG00000102145.15 & GATA1 & 2.768\\
ENSG00000141084.11 & RANBP10 & 2.763\\
ENSG00000100614.18 & PPM1A & 2.757\\
ENSG00000090238.12 & YPEL3 & 2.753\\
ENSG00000232334.1 & RP11\_47G112 & 2.749\\
ENSG00000063854.13 & HAGH & 2.745\\
ENSG00000185883.12 & ATP6V0C & 2.745\\
ENSG00000140564.13 & FURIN & 2.716\\
ENSG00000159346.13 & ADIPOR1 & 2.701\\
ENSG00000257335.8 & MGAM & 2.678\\
ENSG00000137193.14 & PIM1 & 2.660\\
ENSG00000158828.8 & PINK1 & 2.657\\
ENSG00000100558.9 & PLEK2 & 2.657\\
ENSG00000182512.5 & GLRX5 & 2.628\\
ENSG00000135083.16 & CCNJL & 2.626\\
ENSG00000166825.15 & ANPEP & 2.579\\
ENSG00000068971.14 & PPP2R5B & 2.573\\
ENSG00000115590.14 & IL1R2 & 2.566\\
ENSG00000238005.4 & LNCATV & 2.550\\
ENSG00000084110.11 & HAL & 2.534\\
ENSG00000185630.19 & PBX1 & 2.531\\
ENSG00000147454.14 & SLC25A37 & 2.526\\
ENSG00000119326.15 & CTNNAL1 & 2.451\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_rda_weights_prot.tex <==
% Proteins 

\begin{table}
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{0.8}
    \caption{{\bf Stable Proteins Selected by HIP (Random) for the COPDGene Data.} Weights are averages from the estimated $\bm B^{d,s}$ matrices from the subset fit where the variable was selected. Higher values suggest the variable likely contributes more to association and prediction.}\label{ext:tab:rda:proteins}
%\begin{tabular}{clcc}
\begin{tabular}{p{1.25cm}p{7cm}p{1.75cm}p{1cm}}
\toprule
Subgroup & Name & Symbol & Weight\\
\midrule
 & SHC-transforming protein 1:Src Homology domain & SHC1 & 3.174\\
 & Amyloid beta A4 protein & APP & 3.062\\
 & Neutrophil-activating peptide 2 & PPBP & 3.031\\
 & Connective tissue-activating peptide III & PPBP & 3.022\\
 & UDP-glucuronosyltransferase 2A1 & UGT2A1 & 3.021\\
 & SPARC & SPARC & 3.008\\
 & Heparin-binding EGF-like growth factor & HBEGF & 3.003\\
 & Platelet-derived growth factor subunit A & PDGFA & 2.981\\
 & Thrombospondin-1 & THBS1 & 2.899\\
 & Platelet basic protein & PPBP & 2.886\\
 & Endoplasmic reticulum resident protein 44 & ERP44 & 2.809\\
 & Beta-thromboglobulin & PPBP & 2.782\\
 & B-cell antigen receptor complex-associated protein alpha chain & CD79A & 2.742\\
 & Platelet-derived growth factor subunit B & PDGFB & 2.742\\
 & Brain-derived neurotrophic factor & BDNF & 2.738\\
 & Tudor-interacting repair regulator protein & NUDT16L1 & 2.702\\
 & Collagen type IV alpha-3-binding protein:StAR-related lipid-transfer domain, isoform 2 & CERT1 & 2.679\\
 & C-C motif chemokine 5 & CCL5 & 2.665\\
 & Lysyl oxidase homolog 3 & LOXL3 & 2.641\\
\multirow[t]{-20}{*}{\centering\arraybackslash Males} & Syntaxin-8 & STX8 & 2.420\\

\cmidrule{1-4}

 & Amyloid beta A4 protein & APP & 3.655\\
 & UDP-glucuronosyltransferase 2A1 & UGT2A1 & 3.558\\
 & Neutrophil-activating peptide 2 & PPBP & 3.553\\
 & Connective tissue-activating peptide III & PPBP & 3.539\\
 & SHC-transforming protein 1:Src Homology domain & SHC1 & 3.503\\
 & Platelet basic protein & PPBP & 3.392\\
 & Platelet-derived growth factor subunit A & PDGFA & 3.365\\
 & Glia-derived nexin & SERPINE2 & 3.362\\
 & SPARC & SPARC & 3.353\\
 & WAP four-disulfide core domain protein 13 & WFDC13 & 3.286\\
 & Beta-thromboglobulin & PPBP & 3.279\\
 & Heparin-binding EGF-like growth factor & HBEGF & 3.257\\
 & Thrombospondin-1 & THBS1 & 3.229\\
 & Collagen type IV alpha-3-binding protein:StAR-related lipid-transfer domain, isoform 2 & CERT1 & 3.182\\
 & Brain-derived neurotrophic factor & BDNF & 3.164\\
 & Lysyl oxidase homolog 3 & LOXL3 & 3.072\\
 & Peptidyl-prolyl cis-trans isomerase FKBP7 & FKBP7 & 3.052\\
 & Tudor-interacting repair regulator protein & NUDT16L1 & 3.025\\
 & Platelet-derived growth factor subunit B & PDGFB & 3.000\\
\multirow[t]{-20}{*}{\centering\arraybackslash Females} & Syntaxin-8 & STX8 & 2.845\\
\bottomrule
\end{tabular}
\end{table}
